HOPS 361-C's Jet Decelerating and Precessing Through NGC 2071 IR

We present a two-epoch Hubble Space Telescope (HST) study of NGC 2071 IR highlighting HOPS 361-C, a protostar producing an arced 0.2 parsec-scale jet. Proper motions for the brightest knots decrease from 350 to 100 km/s with increasing distance from the source. The [Fe II] and Pa$\beta$ emission line intensity ratio gives a velocity jump through each knot of 40--50 km/s. A new [O I] 63 \mic\ spectrum, taken with the German REciever for Astronomy at Terahertz frequencies (GREAT) instrument aboard Stratospheric Observatory for Infrared Astronomy (SOFIA), shows a low line-of-sight velocity indicative of high jet inclination. Proper motions and jump velocities then estimate 3D flow speed for knots. Subsequently, we model knot positions and speeds with a precessing jet that decelerates. Measurements are matched with a precession period of 1,000--3,000 years and half opening angle of $15^\circ$. The [Fe II] 1.26-to-1.64 \mic\ line intensity ratio determines visual extinction to each knot from 5--30 mag. Relative to $\sim$14 mag of extinction through the cloud from $\rm{C}^{18}$O emission maps, the jet is embedded at a 1/5 to 4/5 fractional cloud depth. Our model suggests the jet is dissipated over a 0.2 pc arc. This short distance may result from the jet sweeping through a wide angle, allowing the cloud time to fill cavities opened by the jet. Precessing jets contrast with nearly unidirectional protostellar jets that puncture host clouds and can propagate significantly further.

==> Other Notes/molecular_h2_s1.tex <==
many molecular observations vs our NIR outflows, different speeds for different atoms, wavelengths?

compare with Av map, uncertainties

Why do H2 and [FeII] behave differently

forward cite Li et al 2013 for any responses about outflow cavities

NIR molecular hydrogen S(1)
Walther 2019 JHK and molecular hydrogen using Gemini North
% https://iopscience.iop.org/article/10.3847/1538-4357/ab0e0b/pdf
Zhao 1999: identifying HH objects with NIR  images and the Beijing Astronomical Observatory
% https://iopscience.iop.org/article/10.1086/301002/pdf
molecular hydrogen transitions (molecular outflows)
Aspin 1992: fabry-perot image of IRS sources and S(1) molecular hydrogen
% https://articles.adsabs.harvard.edu/pdf/1992MNRAS.258..684A
Burton 1989: looks at molecular hydrogen S(1)
% https://articles.adsabs.harvard.edu/pdf/1989MNRAS.238.1513B
Bally 1983 and 1982: looks at atomic hydrogen (21 cm HI) with VLA. They conclude that the HI outflow is not dynamically important around the YSOs and CO is better. The 1982 papers looks at CO and CS as well as the H2 S(1) transition
% https://articles.adsabs.harvard.edu/pdf/1983ApJ...266L..61B
% https://articles.adsabs.harvard.edu/pdf/1982ApJ...261..558B
% https://articles.adsabs.harvard.edu/pdf/1982ApJ...257..612B
Persson 1981: looks at H2 S(1) line emission at approx 2 microns.
% https://articles.adsabs.harvard.edu/pdf/1981ApJ...251L..85P

% FIR observations reorder + difference between different emitting sources in the cloud ... van kempen 2014: organic emission using herschel (HIFI called WISH Key) and SMA (taken in 2010, van kampen 2012 for continuum) *** actually some good ideas, talks about shock desorption in intro to note offsets between organic emissions and outflows (maybe something similar with the collimation of FeII vs H2?) - also see Buckle and Fuller 02? probably beter paper than these for that idea
% https://www.aanda.org/articles/aa/pdf/2014/09/aa23821-14.pdf ...Is neufeld 09 of interest? maybe not?
% Houde 2001 magnetic fields, collimated outflows, and radio emissions
% https://iopscience.iop.org/article/10.1086/318339/pdf
% Kitamura 1990 and 1992: studying CS, HCO+, HCN, argues for wind-driven, expanding dense bubbles  that result in the bipolar outflow seen, its size (?), and clumps (or sub-clumps?). Also tries to apply Rayleigh-Taylor instability
%https://articles.adsabs.harvard.edu/pdf/1990ApJ...363..180K and https://articles.adsabs.harvard.edu/pdf/1992PASJ...44..407K
% Moriarty-Schieven 1989: 12CO maps, tries to explain how motions of stellar wind jet impacts the end wall of the lobe cavity
% Tauber 1988: looks at H2CO spectra and discusses collimation
% https://articles.adsabs.harvard.edu/pdf/1988ApJ...325..846T
% Schwartz 1983: Looks at NGC 1333 and NGC 2071 in C18O, NH3, CS. Argues the jets are snowplowing into the surrounding cloud with high-velocity low-density gas.
% https://articles.adsabs.harvard.edu/pdf/1983ApJ...267L.109S
% https://articles.adsabs.harvard.edu/pdf/1989ApJ...347..358M
% Persson 1981: looks at H2 S(1) line emission at approx 2 microns. Notes some IR sources, suggests a radiatively driven wind?
% https://articles.adsabs.harvard.edu/pdf/1981ApJ...251L..85P

% cavity opening/turbulent entrainment li et al, ...

FIR observations, molecules, and gas mass/chemistry
Liu et al 2020: SOFIA/SOMA, using FORCAST ... has 7, 11, 19, 31, 37 microns and also potentially Spitzer/IRAC and Herschel/PACS
% https://iopscience.iop.org/article/10.3847/1538-4357/abbefb/pdf
Neufeld et al 2014: water abundances from herschel/pacs and spitzer/irs
% https://iopscience.iop.org/article/10.1088/0004-637X/781/2/102/pdf
van kempen 2014: organic emission using herschel and SMA
% https://www.aanda.org/articles/aa/pdf/2014/09/aa23821-14.pdf
Giannini 2011: spitzer line maps (Figure 3 at least is more extended than the ALMA/VLA view, nice for comparison, but it IS IRS primarily for S1 molecular hydrogen and HD, maybe more for discussion)
% https://iopscience.iop.org/article/10.1088/0004-637X/738/1/80/pdf
Melnick 2008 Extended hot water emission using Spitzer
% https://iopscience.iop.org/article/10.1086/589853/pdf
Johnstone 2003: astrochemistry in Orion at sub-mm
% https://www.aanda.org/articles/aa/pdf/2003/47/aa3536.pdf
Butner et al 1990: used KAO to make line profiles
% https://articles.adsabs.harvard.edu/pdf/1990ApJ...364..164B
Scoville 1986: looks at CO, estimates mass flux
% https://articles.adsabs.harvard.edu/pdf/1986ApJ...303..416S
Wootten 1984: calculates hydrogen mass (appendix), looks at HCO+, H13CO+, abundance of HCO+
% https://articles.adsabs.harvard.edu/pdf/1984ApJ...279..633W



and CO/water/other molecules)
Stojimrovic 2008: imaged in 12CO, 13 COJ=1-0 + SCUBA %https://iopscience.iop.org/article/10.1086/586688/pdf 
Seth 2002: H2O masers
% https://iopscience.iop.org/article/10.1086/344225/pdf
Garay 2000: SiO and methanol using SEST
% https://iopscience.iop.org/article/10.1086/317853/pdf
Torrelle 1998: H2O masers, radio continuum
% https://iopscience.iop.org/article/10.1086/306205/pdf
Girart 1997 and 1999: HCO+ molecular outflow
% https://articles.adsabs.harvard.edu/pdf/1997IAUS..182P.123G
Chernin 1993 and 1995: high-velocity CO emission, then SO and SiO, then , CO outflow hot spots?
% https://articles.adsabs.harvard.edu/pdf/1992ApJ...396L..35C
% https://articles.adsabs.harvard.edu/pdf/1993ApJ...403L..21C
% https://articles.adsabs.harvard.edu/pdf/1995ApJ...440L..21C
Goldsmith 1992: CO, 13CO, C18O, CS, HCO+; notes an IRAS source+significant CS emission
% https://articles.adsabs.harvard.edu/pdf/1992ApJ...385..522G
Zhou et al 1990 and 1991: NH3, notes IRS sources, same in 91 but with CS
% https://articles.adsabs.harvard.edu/pdf/1990ApJ...355..159Z
% https://articles.adsabs.harvard.edu/pdf/1991ApJ...372..518Z
Yamashita 1989: CS with JCMT around IRS 1
% https://articles.adsabs.harvard.edu/pdf/1989ApJ...347L..85Y
Takano 1984, 1986: CS, NH3 spectra
% https://articles.adsabs.harvard.edu/pdf/1986ApJ...300L..85T
% https://articles.adsabs.harvard.edu/pdf/1984ApJ...282L..69T
Padman 1982: HCO+ J=4-3
% https://articles.adsabs.harvard.edu/pdf/1982MNRAS.200..183P
Calamai 1982: NH3
% https://articles.adsabs.harvard.edu/pdf/1982A%26A...109..123C
Lichten 1982: looks at CO line profile 
% https://articles.adsabs.harvard.edu/pdf/1982ApJ...253..593L
Campbell 1978: H2O maser
% https://articles.adsabs.harvard.edu/pdf/1978PASP...90..262C
Johansson 1974: OH
% https://articles.adsabs.harvard.edu/pdf/1974ApJ...189..455J

==> Other Notes/outlining.tex <==
***Note group specialties: Dan's is fluids or plasmas/shocks/chemistry, Tom's is statistics of energetics/star clusters/NIR imaging, Alice's is dynamics and mechanics

updating financial info, adding DOIs for data.
*Make sure to submit to star formation newsletter and arxiv when submitted!


==> Other Notes/propmot_methods.tex <==
%TBD for adding: cross-correlation, optical flow, image segmentation...

Methods of determining proper motions for HH objects are often done by finding centroids for boxes of interest overlaid on images \citep{Bally_2002, Reiter_2017, Erkal_2021}, by shifting a window or mask over a knot in one epoch until it reduces the difference with a box over the same knot in another epoch \citep{Hartigan_2001}, by fitting more complex shapes (e.g. a symmetric parabola or Gaussian) to a knot or the jet \citep{Eisloeffel_1992}, or by cross-correlation of both images \citep{Reipurth_1992, Raga_2012, Raga_2017}.  
%Outside these selections, the only more complex methods are used in computer science, computer vision, weather tracking, identifying smoke patterns from images, etc.

Centroids have the advantage of being controllable to a labeled box region or mask, but we found many of our knots change morphology and brightness even when more isolated. Cross-correlation can be less sensitive to the shape and size of region chosen, but it is also difficult to remove bright features or noise even when normalizing an image or applying background subtraction. 
%I remember someone discussing virtual knots, but I can't remember where ... also note how cross-correlation can lead to "virtual knots"

% Next, we measured moving features in the image using cross-correlation \citep[e.g.]{GarciaDiaz_2015}. We identified bright knots of interest by blinking the two images with SAO DS9. We checked this against \red{add some references below from "ideas for blobs to mark"}. 

% We enclosed each knot in a box region in the difference image to capture emission between the two frames. We then autocorrelated the F160W image and cross-correlated the epoch 1 and synthetic epoch 2 images. This gives a bright peak between epoch 1 and epoch 2 that gives at minimum single pixel shifts. 

Similar to \citep{Erkal_2021} we have opted for identifying knots from the difference image. While simple, visually locating the brightest pixel captures a sensible decreasing trend in tangential velocities for knots expected along the HOPS 361-C outflow in Table \ref{tab:propmot}. This further gives the capability to model precession, one of our main scientific results.

% While there is a long history of using cross-correlations to determine movement in images, there is criticism over how to precisely choose the correct box region or window or knot \red{will add some papers from below, likely Hartigan 01?}. 

%this is just to note some references for what I may compare with...
% how to measure proper motions with cross-correlation
% Garcia Diaz et al 2015
% https://iopscience.iop.org/article/10.1088/0004-637X/798/2/129/pdf
% reipurth 92
% https://articles.adsabs.harvard.edu/pdf/1992ApJ...392..145R
% lopez 96 
% https://articles.adsabs.harvard.edu/pdf/1996MNRAS.282..470L
% Anglada et al 07: using cross-correlation
% https://iopscience.iop.org/article/10.1086/517493/pdf and  https://ui.adsabs.harvard.edu/abs/2007AJ....133.2799A/citations for reference

% \red{TBD: may add more on my other options=skimage/skeletonize, trackpy, and openpiv}. Centroids can provide sub-pixel accuracy, but they can involve oversampling or identifying unrealistic or subjective patterns. For our purposes, provide brightness-weighted centroids (https://photutils.readthedocs.io/en/stable/centroids.html) for both F160W images as a simple and intuitive check. Subtracting the two centroids provides a shift for each boxed-in knot. 
% Pixel shifts and minimizing overlaps
% (eta car currie 96) 
% https://articles.adsabs.harvard.edu/pdf/1996AJ....112.1115C 
% eta car 01 (morse)
% https://iopscience.iop.org/article/10.1086/319092/pdf
% Hartigan HH objects 01
% https://iopscience.iop.org/article/10.1086/323976/pdf
% bally 2002
% https://iopscience.iop.org/article/10.1086/339837/pdf

%last option is GarciaDiaz_2015

==> knots_tan_vels.tex <==
% A jet curved or deflected by surrounding material is not supported by our proper motion directions. A collision or nearby partner jerking the jet from HOPS 361-C cannot be ruled out. But there are other nearby stars in the HOPS 361 region, such as HOPS 366 and 335. This may be the cause of some scatter in the velocities we observe.

%But the timescale for a 100 km/s jet ejected out to 0.1 pc must be on the order of 1000 years, 
% We do not have detailed observations for those HOPS sources or data to measure the velocity dispersion of stars in the region to determine a collisional timescale, but the probability for collisions would be proportional to the ratio of a star's volume to the volume of the cloud its embedded in. 
% Considering that protostars like HOPS 361-C is less than 1 arcsec in size, while the HOPS 361 region its embedded in is about 20 arcsec in size, then taking these regions as spherical, there would be a 0.01\% chance of colliding with another stars on average. Considerations towards the impact parameter required would make this less likely, but it still cannot be ruled out as their are nearby protostars in the region.

% HOPS 335 is a protostellar source in the center of the jet and may be related to a velocity driven up and out of the general region of flow, but that cannot be ascertained without radial velocities.
% Instead, we proceed by interpreting the proper motions in terms of variations in the jet velocity at its source. 
% For example, the arc and any variations in the ballistic motions may be due to orbital motion in a binary, from precession of the jet's axis, or precession of the orbital axis of the system \citep{Masciadri_2002,Anglada_2007}.

% other options for plots ... 
% Erkal 21: more modern version (but not rigorous)
% https://iopscience.iop.org/article/10.3847/1538-4357/ac06c5/pdf
% Rodriguez-Kamenetsky 22: another modern version (shows nice presentation of motions), more focused on inner portions of jet, though
% https://iopscience.iop.org/article/10.3847/2041-8213/ac6fd1/pdf

% If any comparisons to check are necessary then see...Measured proper motions for NGC 2071 (even if at other wavelengths):
% Gorschedle, Alves, Meingast 2021: using GAIA DR2 to measure proper motions of gas (via YSO tracking?)
% https://www.aanda.org/articles/aa/pdf/2021/03/aa38913-20.pdf
% Carrasco-Gonzalez 2012: VLA and CARMA, also studying YSO SEDs
% https://iopscience.iop.org/article/10.1088/0004-637X/746/1/71/pdf
% Trinidad 2009: radio jets and the VLA
% https://iopscience.iop.org/article/10.1088/0004-637X/706/1/244/pdf
% Seth 2002: H2O masers
% https://iopscience.iop.org/article/10.1086/344225/pdf

% A list of ideas for figure/math presenting based off Anglada et al:
% https://iopscience.iop.org/article/10.1088/2041-8205/720/1/L119/pdf
% https://iopscience.iop.org/article/10.1088/0004-637X/721/2/929/pdf
% https://iopscience.iop.org/article/10.3847/0004-637X/818/1/27/pdf
% https://iopscience.iop.org/article/10.3847/0004-637X/832/2/152/pdf
% http://www.astroscu.unam.mx/rmaa/RMxAA..53-2/PDF/RMxAA..53-2_araga-II.pdf
% R. Lopez et al 2015 3D Kinematics of the near-IR HH 223 outflow in L723
%https://iopscience.iop.org/article/10.1088/0004-6256/144/2/61/pdf
% https://iopscience.iop.org/article/10.1088/0004-637X/713/2/731/pdf
% Tambovsteva and Grinin 2008 Disc wind in the HH 30 binary models


